Spectral-DP: Differentially Private Deep Learning through Spectral Perturbation and Filtering

Differential privacy is a widely accepted measure of privacy in the context of deep learning algorithms, and achieving it relies on a noisy training approach known as differentially private stochastic gradient descent (DP-SGD). DP-SGD requires direct noise addition to every gradient in a dense neural network, the privacy is achieved at a significant utility cost. In this work, we present Spectral-DP, a new differentially private learning approach which combines gradient perturbation in the spectral domain with spectral filtering to achieve a desired privacy guarantee with a lower noise scale and thus better utility. We develop differentially private deep learning methods based on Spectral-DP for architectures that contain both convolution and fully connected layers. In particular, for fully connected layers, we combine a block-circulant based spatial restructuring with Spectral-DP to achieve better utility. Through comprehensive experiments, we study and provide guidelines to implement Spectral-DP deep learning on benchmark datasets. In comparison with state-of-the-art DP-SGD based approaches, Spectral-DP is shown to have uniformly better utility performance in both training from scratch and transfer learning settings.

==> background.tex <==
\section{Preliminary}\label{sec:prelim}
In this section, we provide a brief background on differential privacy and DPSGD. 
In this work, we study the differentially private perturbation of the gradient descent in the neural network training with model compression. We first provide the basic definition of differential privacy and DPSGD. As we focus on the network with block circulant weight matrices, we provide preliminaries on how block circulant weight matrices works in the fully connected layer.

\subsection{Differential Privacy}
Differential privacy \cite{DP_algorithm} is a privacy definition that describes the privacy loss associated with application who utilizes from a database. It is defined on adjacent databases. We say two databases are adjacent if they differ only in a single entry. Hence, the different privacy is defined by
\begin{definition}\label{def:dp}
    A randomized algorithm $\mathcal{M}$ with domain $\mathcal{D}$ and $\mathcal{R}=\text{Range}(\mathcal{M})$ is $(\epsilon, \delta)-$differentially private if for all $S\subseteq\mathcal{R}$ and for any two adjacent sets $d,d'\in\mathcal{D}$:
    \begin{equation}\label{eq:dp_definition}
        \text{Pr}[\mathcal{M}(d)\in S]\leqslant \exp ^\epsilon \text{Pr}[\mathcal{M}(d')\in S] + \delta
    \end{equation}
\end{definition}
A common mechanism that achieve differential privacy is the Gaussian mechanism. Gaussian mechanism takes as input a sequence $Q$ with $l_2$ sensitivity S and a parameter $\sigma$ controlling the Gaussian noise.  The Gaussian mechanism is formulated as noise perturbation in the output of the sequence:
\begin{equation}\label{eq:GaussianMechanism}
    Gauss(Q,S,\sigma) \triangleq Q + \mathcal{N}(0,S^2\cdot\sigma^2)
\end{equation}
where $\mathcal{N}(0,S^2\cdot\sigma^2)$ is the Gaussian distribution with zero mean and variance $S^2\cdot\sigma^2$. It is noticed that the noise scale in Gaussian mechanism is proportation to the $L_2$ sensitivity. According to Theorem 3.22 in \cite{DP_algorithm}, for any $\epsilon,\delta\in(0,1)$, the Gaussian mechanism achieve $(\epsilon,\delta)-$differential privacy when $\sigma=\sqrt{2\log(1.25/\delta)}/\epsilon$.
\subsection{DP-SGD and RDP composition}
Differentially private stochastic gradient descent (DPSGD) introdcue differential privacy into deep learning by controlling the influence of the training data during the training process. Specifically in each training iteration, the per-example gradients $g$ with respect to the loss function $L$ is bounded by $l_2$ norm clipping with a threshold $C$. The Gaussian mechanism adds random noise $\calN(0,\sigma^2C^2\mathbb{I})$ into $\sum_{x_{i}\in \cal D}g(x_i)$ to perturb the gradients. The differential privacy of DP-SGD in a single iteration is guaranteed by the Gaussian mechanism. 
The composition property of the differential privacy allows us to compute the overall differential privacy for multiple training iterations. We note that \cite{RDP2017,RDP2019} provide the tightest privacy accountant analysis of the DP-SGD which is based on the R{\'{e}}nyi differential privacy (RDP). The RDP is defined by
\begin{definition}\label{def:RDP}
    A randomized algorithm $\mathcal{M}$ with domain $\mathcal{D}$ and $\mathcal{R}=\text{Range}(\mathcal{M})$ is $(\epsilon, \delta)-$RDP if for any two adjacent sets $d,d'\in\mathcal{D}$:
    \begin{equation}\label{eq:RDP_definition}
        D_{\alpha}(\calM(d)\|\calM(d'))\leqslant \epsilon
    \end{equation}
\end{definition}
where $D_{\alpha}(\cdot\|\cdot)$ is the R{\'{e}}nyi divergence between two probability distributions. More detailed, it is defined by
\begin{definition}\label{def:RenyiDiver}
    For two probability distributions $P$ and $Q$ defined on $\calX$ over the same space, and let $p$ and $q$ denote the densities of $P$ and $Q$ ,respectively, the  R{\'{e}}nyi divergence of order $\alpha>1$ is given by
    \begin{equation}\label{eq:Renyi-divergence_definition}
        D_{\alpha}(P\|Q)\triangleq\frac{1}{\alpha-1}\log\mathop\mbbE\limits_{x\thicksim Q}(\frac{P(x)}{Q(x)})^{\alpha}
    \end{equation}
\end{definition}

Proposition 1 in \cite{RDP2017} provides theoretical foundation of composing RDP mechanisms. In detail, for a mechanism $\calM_1$ with ($\alpha,\epsilon_1$)-RDP and another mechanism $\calM_2$ with ($\alpha,\epsilon_2$)-RDP, then the mechanism $(\calM_1,\calM_2)$ satisfies $(\alpha,\epsilon_1+\epsilon_2)$-RDP. And we note that the RDP mechanism can be converted into the DP using the proposition 3 in \cite{RDP2017} which indicates that an ($\alpha,\epsilon$)-RDP mechanism satisfies ($\epsilon+\frac{\log 1/\delta}{\alpha-1}, \delta$)-DP for any $\delta\in(0,1)$.

% \todo[inline]{Composition RDP}
% \wen{You shouldn't put the algorithm of DP-SGD in the background section, instead, just describe it at a high level. Usually you put only present your own algorithm like this. Also, background should be just some information necessary for readers to understand your technique, not everything.}
% \begin{algorithm}[h]
%     \caption{DPSGD}
%     \label{alg:dpsgd}
%   \begin{algorithmic}[1]
%     \REQUIRE Data entries $\{x_1,\cdots,x_N\}$, loss function $L(\theta)=\frac{1}{N}\sum_{i}L(\theta,x_i)$, learning rate $\eta_t$, noise scale $\sigma$, group size $L$, gradient norm bound $C$\\
%     \STATE \textbf{Initialize} $\theta_0$ randomly
%     \FOR{$t\in[T]$}
%     \STATE Sample a random group $L_t$ with sampling probability $L/N$
%     \STATE For each $x_i\in L_t$, compute $g_t(x_i)\leftarrow\nabla_{\theta_t}L(\theta_t,x_i)$
%     \STATE Clip gradients: $\bar{g}_t(x_i)\leftarrow g_t(x_i)/\max(1,\frac{\|g_t(x_i)\|_2}{C})$\\
%     {\fontfamily{qcr}\selectfont Gaussian Mechanism:}\\
%     \STATE Add noise into average gradient using Gaussian mechanism:
%     $\tilde{g}_t(x_i)\leftarrow\frac{1}{L}(\sum_i\bar{g}_t(x_i)+\mathcal{N}(0,\sigma^2C^2\textbf{I}))$
%     \STATE Gradient descent: $\theta_{t+1}\leftarrow\theta_t-\eta_t\tilde{g}_t$
%     \ENDFOR\\
%     \textbf{Output:} $\theta_T$ with the total privacy cost $(\epsilon,\delta)$ using privacy composition.
%   \end{algorithmic}
% \end{algorithm}

% The differential privacy budget $(\epsilon,\delta)$ is related to the privacy accounting algorithm. We note that \cite{RDP2017,RDP2019} provide the tightest privacy accountant analysis of the DP-SGD which is based on the R{\'{e}}nyi differential privacy.

\subsection{Fourier Transform}
\ourmethod takes Discrete Fourier Transform (DFT) as a tool which transforms data to spectral domain. We provides the primitive of the unitary DFT that does not change the norm. The 1D Discrete Fourier Transform (1D-DFT) transforms a sequence of $N$ numbers $\{x_n\}:=x_0, x_1, \cdots, x_{N-1}$ into another sequence of complex numbers, $\{X_k\}:=X_0, X_1,\cdots,X_{N-1}$. The transformation of $x_n$ is given by
$$X_k=\frac{1}{\sqrt{N}}\sum_{n=0}^{N-1}x_n\cdot e^{-\frac{j2\pi}{N}kn}$$
The inverse DFT is defined by
$$x_n=\frac{1}{\sqrt{N}}\sum_{k=0}^{N-1}X_k\cdot e^{\frac{j2\pi}{N}kn}$$
We say $X_k$ as the $k-$th coefficient in the spectral domain. For convenience, we write $X^N=DFT(x^N)$ as the DFT of a given sequence $\{x_n\}$, and $x^N=IDFT(X^N)$ as the inverse DFT of the obtained DFT coefficients.

The 2D Discrete Fourier Transform (2D-DFT) transforms a 2-dimensional sequence of $N\times N$ with the following 
$$X_{k_1,k_2}=\frac{1}{N}\sum_{n_2=0}^{N-1}\sum_{n_1=0}^{N-1}x_{n_1,n_2}\cdot e^{-\frac{j2\pi}{N}(k_1 n_1+k_2 n_2)}$$
where $X_{k_1,k_2}$ is the 2D DFT coefficients. The inverse 2D-DFT is defined by
$$x_{n_1,n_2}=\frac{1}{N}\sum_{k_2=0}^{N-1}\sum_{k_1=0}^{N-1}X_{k_1,k_2}\cdot e^{\frac{j2\pi}{N}(k_1 n_1+k_2 n_2)}$$

% \subsection{Block Circulant Matrix}\label{subsec:bcm}
% \wen{I feel the background is too lengthy and contains too much information. You might want to move the block-circulant matrix to the design part, instead of background. Again, why you would like to put the algorithm here.}



% The method for applying block circulant matrix into neural network has been well illustrated in \cite{cirCNN_Ding,blockcirculant_1}. Particularly in the fully connected layer, when the weight matrix is block circulant, the forward propagation of the layer can be expressed as the process of “FFT$\longrightarrow$Element-wise Multiplication$\longrightarrow$IFFT”. Algorithm  “FFT$\longrightarrow$Element-wise Multiplication$\longrightarrow$IFFT” operation by using the circular convolution theorem. 
% \begin{algorithm}[h]
%     \caption{Forward propagation of fully connected layer with block circulant weight matrix.}
%     \label{alg:forward_FC_BCM}
%   \begin{algorithmic}[1]
%     \REQUIRE $w_{i,j}$, $x$, $p$, $q$,$k$\\
%     \textbf{Output: } layer activation $a$\\
%     \STATE Initialize the $a$ with zeros
%     \FOR {$i\in 1,2,\cdots,p$}
%     \FOR {$j\in 1,2,\cdots,q$}
%     \STATE $a_i\leftarrow a_i+\text{ifft}(\text{fft}(w_{i,j})\circ \text{fft}(x_j))$
%     \ENDFOR
%     \ENDFOR
%     \STATE \textbf{Return} $a$
%   \end{algorithmic}
% \end{algorithm}
% Given the block circulant matrix $W$ and an input $x\in\mathbb{R}^n$, the computation of the fully connected layer is $a=\psi(W*x)$. For each circulant matrix $W_{i,j}$, the corresponded $a_j$ can be computed by $a_j=W_{i,j}*x_j=\text{ifft}(\text{fft}(w_{i,j})\circ \text{fft}(x_j))$, where $x_j$ is the partition of the input. $x=\{x_0,\cdots,x_j,\cdots,x_q\}$ and $\circ$ is the operation of element-wise multiplication. Hence, the forward propagation process in the fully connected layer is formulated in the Algorithm \ref{alg:forward_FC_BCM}. And the backward propagation process also follows the operation rule “FFT$\longrightarrow$Element-wise Multiplication$\longrightarrow$IFFT”. The backward propagation is formulated in the Algorithm \ref{alg:backward_FC_BCM}
% \begin{algorithm}[h]
%     \caption{Backward propagation of block-circulant matrix-based FC layer.}
%     \label{alg:backward_FC_BCM}
%   \begin{algorithmic}[1]
%     \REQUIRE $\frac{\partial L}{\partial a}$,$w_{i,j}$, $x$, $p$, $q$,$k$\\
%     \textbf{Output: } $\frac{\partial L}{\partial w_{i,j}}$, $\frac{\partial L}{\partial x}$\\
%     \STATE Initialize $\frac{\partial L}{\partial w_{i,j}}$, $\frac{\partial L}{\partial x}$ with zeros
%     \FOR {$i\in 1,2,\cdots,p$}
%     \FOR {$j\in 1,2,\cdots,q$}
%     \STATE $\frac{\partial L}{\partial w_{i,j}}\leftarrow \text{IFFT}(\text{FFT}(\frac{\partial L}{\partial a_{i}})\circ \text{FFT}(x'_j))$
%     % \STATE $\frac{\partial L}{\partial x_{j}}\leftarrow \frac{\partial L}{\partial x_{j}}+\text{ifft}(\text{fft}(\frac{\partial L}{\partial a_{i}})\circ \text{fft}(w_{i,j}))$
%     \ENDFOR
%     \ENDFOR
%     \STATE \textbf{Return} $\frac{\partial L}{\partial w_{i,j}}$, $\frac{\partial L}{\partial x}$
%   \end{algorithmic}
% \end{algorithm}


==> motivation.tex <==
\section{Motivation}
It is incontestable that neural networks become more redundant as the networks tend to be deeper and deeper. To simplify the neural networks, pruning is introduced to reducing the redundancy. The key idea of pruning is to remove neurons or parameters. Most pruning methods focus on removing neurons or parameters (near zero weights), and such methods are conducted on the spatial domain. Since pruning is a natural way to providing less variation, we explore if pruning can be applied into the gradient. Due to gradient contains much information, directly pruning the gradient on the signal or time domain causes a huge utility loss. We then focus on the pruning that is conducted on the spectral domain.

Consider a neural network that only contains convolution layers, the gradient of each convolution filter can be expressed an multiplication on the spectral domain by implementing Fourier transform. The spectral pruning removes the relatively unimportant spectral coefficients, and the resulting gradient is expressed as the inverse Fourier transform of the pruned spectral coefficients. We implement the network on the CIFAR-10 dataset with spectral pruning. The results show that the accuracy drop is small compared to the un-pruned network.

As the noise is added into the gradient to ensure the privacy guarantee, pruning the noisy gradient is a natural way to decreasing the scale of the noise. Due to gradient contains much information, directly pruning the gradient on the signal or time domain causes a huge utility loss. 

To overcome it, we explore how to conduct such pruning on the spectral domain. We note there are spatial redundancies on the convolution filers. Hence, pruning on the spectral domain  

we then explore the idea of Based on that, we explore how pruning works on we focus on the gradient pruning and how to conduct such pruning on the spectral domain.

We note there are spatial redundancies on the convolution filters, and we explore the spectral pruning The spectral pruning is achieved by pruning away unimportant spectral gradients. Specifically, it is implemented by 
To implement pruning on the differentially private training process, the noisy gradients are set to be zeros 

We note set weights as zeroPruning 

which The objective of 
The pruning methods are based on the spatial domain. Consider a scenario 
Since convolutional neural networks tend to be deeper and deeper which means more storage requirements and floating-point operations, there are many works devoting to simplify and accelerate the deep neural networks.
Due to the high dimensional data requires a larger neural network with more layers and nodes, reducing the memory cost and the computational is critical in the practical application. Model compression methods such as quantization, pruning, and structured weight matrix are widely used in reducing the complexity of deep learning model with little loss of accuracy. Bock circulant weight matrix is introduced in \cite{cirCNN_Ding,blockcirculant_1} to reduce the redundancy of the parameters in fully connected layer. The block circlulant matrix allows the use of Fourier transformation in the backward propagation. Based on this, we propose a differentially private perturbation in the architecture that contains fully connected layer with block circulant weight matrix. The proposed method utilizes the block circulant matrix as a dimension "reduction". And the key idea is that we first perturb the gradient in the Fourier domain then apply a Fourier filtering mechanism to limit the space of weights, thus resulting fewer noise variables to add in the training. 


==> revision_plan.tex <==
\title{Cover Letter}
% \maketitle

% We thank the reviewers for the careful reading and comments, and the shepherd for the help in improving the quality of the paper. Below we provide our revision plan, and summarize the corresponding revisions we have made in the updated paper. For your convenience, we provide an annotated version of our revised paper, in which only the changes required in this round are marked in {\color{red} red}. 

% \section{Reviewer A}

% \textbf{P1: Complexity.} We include theoretical analysis of the complexity of FFT-based convolution in Section~\ref{subsec:conv_spectral_dp} and the complexity analysis of block circulant matrices (BCM) based FC layer in Appendix \ref{apdx:complexity}.

% \textbf{P2: Filtering ratio impact.} As pointed out in the  rebuttal, we have included a study of the filtering ratio on CIFAR10 (see Section~\ref{subsec:effectiveness_spectral_dp} and Table~\ref{tab:conv1-pruning}).  
% In the revision, We provide more results of filtering ratio impact on CIFAR10 in Appendix \ref{appdix:ablation_cifar_transfer} and CIFAR100 in Section~\ref{subsec:transfer_learning_ablation}.

% \textbf{P3: Lossless transform.} We correct the statement as advised by the reviewer in Section~\ref{sec:relatedwork}.



% \section{Reviewer B}

% \textbf{P1: Limitations/Shortcomings. }
% We add Section~\ref{sec:limitations} to discuss the limitations.
% As discussed in the rebuttal, there still exists the utility or accuracy gap for deep models that are trained from scratch, and there’s scope to explore other possible domain transformation techniques in addition to DFT along this direction. We also discuss the areas for the future improvement of Spectral-DP.  



% \section{Reviewer C}

% \textbf{P1: Comparison Spectral-DP against other works and De et al “DeepMind”.} As suggested by the reviewer, we have run additional experiments on CIFAR10 and CIFAR100 and compared Spectral-DP with more recent baselines including DeepMind~\cite{de2022unlocking}, AAAI21~\cite{papernot2021tempered}, ICLR21~\cite{tramer2021differentially} in Section~\ref{subsec:WRN_transfer}.

% \textbf{P2: Comparison against Luo et al. CVPR2021.} We include the results of ResNeXt compared to this work, as shown in our rebuttal.
% This has been added to Appendix~\ref{appendix:transfer_resnext} due to space limitations.
% % in Appendix \ref{appendix:transfer_resnext} due to space limitation. 

% \textbf{P3: Cases/settings where this lost information significantly hurts utility.} We discuss these cases in Section~\ref{sccratch} and Section~\ref{subsec:transfer_learning_ablation}.


% \section{Reviewer D}

% \textbf{P1: Privacy composition and sampling technique.} 
% In Section~\ref{sec:DPtogether},
% we add the information regarding the sampling operation into Algorithm~\ref{alg:PutInDL}.
% % we added the sampling step in Algorithm~\ref{alg:PutInDL}.
% We clarify the sampling technique with the supporting reference in the second paragraph of Section~\ref{sec:DPtogether}.
% We also modify Corollary~\ref{cor:composition} accordingly.
% % We addressed these issues in the rebuttal as the reviewer suggested. In the revision, we will provide and clarify the privacy composition technique and cite the related materials. We will also clarify the sampling method in Section 3.4 and modify Algorithm 4 and Corollary 2 accordingly. 

% \textbf{P2: Experiments of standard architecture.} We have conducted additional experiments that demonstrate the effectiveness of Spectral-DP by using standard neural networks architectures including Wide-ResNet and ResNeXt. In the revised manuscript, we update the results in Section~\ref{subsec:WRN_transfer} and Appendix \ref{appdix:ablation_cifar_transfer}, respectively.

% \textbf{P3: Concentrating the weights in the low bandwidth domain.} 
% In Section~\ref{sec:introduction}, we provided the corresponding justification supported by relevant references for concentrating weights in the low bandwidth region. 
% % We add the motivation of concentrating on low bandwidth in Section~\ref{sec:introduction} with references.


% \section{Additional modifications}
% \begin{enumerate}
% \item In Section~\ref{sec:introduction}, we modified the contribution and the organization of the paper as we added additional experimental results and Section~\ref{sec:limitations} in the revision.
% \item In Section~\ref{sec:approach}, to avoid confusion caused by using time domain and signal domain interchangeably, we replace time domain by spatial domain.
% \item  In Section~\ref{subsec:theoreticalanalysis}, we move the proof of Proposition 3 to Appendix \ref{Appendix:noise_reduction} due to the space limit.
% \item In Section~\ref{subsec:adaptingspectralDPin2dconv}, we move the proof of Corollary 1 to Appendix \ref{Appendix:noise_reduction2D} due to the space limit.
% \item The original content in Section~\ref{subsec:transfer_learning_ablation} about the ablation study on CIFAR10 transfer models is moved to Appendix \ref{appdix:ablation_cifar_transfer} due to the space limit.

% \end{enumerate}



We thank you for the time and effort in reviewing our revision and providing valuable comments. We have carefully considered the comments and provided a response to address each of the concerns. 

\section{Comment 1: Privacy guarantee in Cor. 2}

We clarify that the experimental number of privacy accounting does not change. All privacy accounting is based on the sampling technique in \cite{2019arXiv190810530M}. 

We are sorry for the confusion, in the prior submission, \textbf{$T$} represents the \textbf{total training iterations} of Spectral-DP. 
To avoid confusion, in this revision, we define $T_e$ as the \textbf{training epochs} of Spectral-DP. 
% In this revision, we clarified the sampling technique in Algorithm 4 and used \textbf{T to represent the training epochs} of Spectral-DP. 
As the number of \textbf{total training iterations} is computed as the product of training epochs and $N/B$ ($N$ is the size of the training dataset, $B$ is the batch size), we modified Corollary 2 by replacing $T$ with $T_e*(N/B)$. 


\section{Comment 2: Result of ResNeXt}
We have moved the result of ResNeXt to Section \ref{subsec:transfer_resnext} in the revised draft. We added Table~\ref{tab:apdx-transfer} and marked the new content in {\color{red} red}. 




